Mixed $\mathcal{H}_2/\mathcal{H}_\infty$-Policy Learning Synthesis

A robustly stabilizing optimal control policy in a model-free mixed $\mathcal{H}_2/\mathcal{H}_\infty$-control setting is here put forward for counterbalancing the slow convergence and non-robustness of traditional high-variance policy optimization (and by extension policy gradient) algorithms. Leveraging It\^{o}'s stochastic differential calculus, we iteratively solve the system's continuous-time closed-loop generalized algebraic Riccati equation whilst updating its admissible controllers in a two-player, zero-sum differential game setting. Our new results are illustrated by learning-enabled control systems which gather previously disseminated results in this field in one holistic data-driven presentation with greater simplification, improvement, and clarity.

==> sections/alg_mf.tex <==
\section{Iterative GARE Solver}

We know that the differential game admits equal upper and lower values because the GARE \eqref{eq:lq_two_player} admits a positive definite solution~\citep[Th 4.8 (iii)]{BasarBook} given by $\mc{J}^\star = x^T P x$. Thus, along the trajectories of \eqref{eq:system}, the derivative of $x^TPx$  (using It\^{o}'s formula) can be verified to be (see \citep[\S IV]{CuiMoluxTAC})
%
\begin{align}
	\begin{split}
		&d(x^TPx) = x^T(A^TP + PA)xdt + 2x^T PBu dt \\
		&\qquad + 2x^T P Ddw + \text{Tr}(D^T P D) dt.
		\label{eq: derivative xPx}
	\end{split}
\end{align}


\begin{algorithm}
	\caption{Mixed $\mathcal{H}_2/\mathcal{H}_\infty$-Control Synthesis \label{alg:mixed_synthesis}}
	\begin{algorithmic}
		\State Initialize $\hat{K}_{1} \in \mathcal{K}$
		\Comment{\footnotesize{\eg searching for a valid CLF~\cite{Weehong2006}}}; 
		%
		\State  Collect data from (\ref{eq: LTI with disturbance}) with exploratory input (\ref{eq: exploration input}); and 
		%
		\State Construct matrices $\hat{\Phi}(t_f)$ and $\hat{\Psi}(t_f)$; 
		%
		\For{$i \leq \bar{i}$}
		\For{$j \leq \bar{j}$}
		\State Construct the matrices $\hat{\Lambda}_i^j(t_f)$ using %\eqref{eq:alpha};
		%
		\State Calculate $\hat{P}_{K_i}^j$ using %(\ref{eq: solve P by data});
		%
		\State Update $\hat{L}_{K_i}^j = \gamma^{-2}D^T\hat{P}_{K_i}^j$;
		%
		\State Form $vec^T(\widehat{B^T{P}_{K_i}^{\bar{j}}})$ as $[\hat{\Phi}^{-1}(t_f)]_{n_1+1:n_2} \hat{\Xi}(t_f) vecs(\hat{P}_{K_i}^{\bar{j}})$;
		%
		\State Calculate $\hat{K}_{i+1} = R^{-1} \widehat{B^T{P}_{K_i}^{\bar{j}}}$;
		\EndFor
		\EndFor
	\end{algorithmic}
	%
\end{algorithm}

